On choosing optimal response transformations for dimension reduction

It has previously been shown that response transformations can be very effective in improving dimension reduction outcomes for a continuous response. The choice of transformation used can make a big difference in the visualization of the response versus the dimension reduced regressors. In this article, we provide an automated approach for choosing parameters of transformation functions to seek optimal results. A criterion based on an influence measure between dimension reduction spaces is utilized for choosing the optimal parameter value of the transformation. Since influence measures can be time-consuming for large data sets, two efficient criteria are also provided. Given that a different transformation may be suitable for each direction required to form the subspace, we also employ an iterative approach to choosing optimal parameter values. Several simulation studies and a real data example highlight the effectiveness of the proposed methods.

==> references.bib.tex <==
@article{heng2001study,
  title={A study of sensitivity analysis on the method of principal {H}essian directions},
  author={Lue, H.-H.},
  journal={{Comput. Stat.}},
  volume={16},
  number={1},
  pages={109--130},
  year={2001},
  publisher={Springer}
}

@article{Hampel74,
 ISSN = {01621459},
 URL = {http://www.jstor.org/stable/2285666},
 author = {F. R. Hampel},
 journal = {{J}. {A}m. {S}tat. {A}ssoc.},
 pages = {383-393},
 publisher = {[American Statistical Association, Taylor & Francis, Ltd.]},
 title = {The Influence Curve and Its Role in Robust Estimation},
 volume = {69},
 year = {1974}
}% number = {346},

@article{box1964analysis,
  title={An analysis of transformations},
  author={Box, G. E.P. and Cox, D. R},
  journal={{J}. {R}. {S}tat. {S}oc.: {S}eries {B} (Methodological)},
  volume={26},
 
  pages={211--243},
  year={1964},
  publisher={Wiley Online Library}
}% number={2},

@phdthesis{GarnhamAlexandraLouise2014Imdr,
year = {2014},
title = {Improving modern dimension reduction methods through transformations},
journal = {PhD dissertation},
author = {Garnham, A. L.},
}%Alexandra Louise

@Article{stein1981,
  author    = {Stein, C. M.},
  title     = {Estimation of the Mean of a Multivariate Normal Distribution},
  journal   = {{A}nn. {S}tat.},
  year      = {1981},
  volume    = {9},
  pages     = {1135--1151},
  doi       = {10.1214/aos/1176345632},
  file      = {:References/Stein(1981).pdf:PDF},
  fjournal  = {The Annals of Statistics},
  publisher = {The Institute of Mathematical Statistics},
  url       = {http://dx.doi.org/10.1214/aos/1176345632},
}%  number    = {6},   month     = {11},

%DR
@article{BR83,
  AUTHOR =       {Brillinger, D. R.},
  YEAR = {1983},
  TITLE =        {A genralized linear model with ``{G}aussian" regressor variables},
  JOURNAL = {{A} {F}estschrift For {E}ric {L}. {L}ehmann, {W}adsworth {S}tatist. /{P}robab. {S}er. {B}elmont, {CA}: {W}adsworth},
  PAGES = {97-114},
}%P.J. Bickel, K.A. Doksum, J.L. Hodges (Eds.), International Group,

@article{Li91,
author = { K.-C.   Li },
title = {Sliced Inverse Regression for Dimension Reduction},
journal = {{J}. {A}m. {S}tat. {A}ssoc.},
volume = {86},
pages = {316-327},
year = {1991},
doi = {10.1080/01621459.1991.10475035},
}%number = {414},

@article{Li92,
    author = {Li, K.-C.},
    citeulike-article-id = {1910109},
    citeulike-linkout-0 = {http://dx.doi.org/10.2307/2290640},
    citeulike-linkout-1 = {http://www.jstor.org/stable/2290640},
    doi = {10.2307/2290640},
    issn = {01621459},
    journal = {{J}. {A}m. {S}tat. {A}ssoc.},
    keywords = {hessian, sampling, statistics},
    pages = {1025--1039},
    posted-at = {2009-07-18 00:41:34},
    priority = {0},
    publisher = {American Statistical Association},
    title = {{On Principal Hessian Directions for Data Visualization and Dimension Reduction: Another Application of Stein's Lemma}},
    url = {http://dx.doi.org/10.2307/2290640},
    volume = {87},
    year = {1992}
}%    number = {420},

@Book{Cook98,
    Author = {R. D. Cook},
    Title = {{Regression graphics. Ideas for studying regressions through graphics.}},
    ISBN = {0-471-19365-8},
    Pages = {xviii + 349},
    Year = {1998},
    Publisher = {New York: {J}ohn {W}iley \& {S}ons {I}nc.},
    Language = {English},
    MSC2010 = {62-09 62-01 62J99},
    Zbl = {0903.62001}
}


@Book{Rudolf,
    author = {R. Enz},
    Title = {{Prices and Earnings Around the Globe}},
    Year = {1991},
    publisher = { {Z}urich: {U}nion {B}ank of {S}witzerland}
}

@article{Cook98a,
 ISSN = {01621459},
 URL = {http://www.jstor.org/stable/2669605},
 abstract = {Li has suggested the method of principal Hessian directions for estimating plotting directions that capture curvature in regression functions. This article revisits Li's proposal, offering a number of suggestions for improved application.},
 author = {R. D. Cook},
 journal = {{J}. {A}m. {S}tat. {A}ssoc.},
 pages = {84--94},
 publisher = {[American Statistical Association, Taylor & Francis, Ltd.]},
 title = {Principal Hessian Directions Revisited},
 volume = {93},
 year = {1998}
}%number = {441},



@article{Smith10,
 ISSN = {03036898, 14679469},
 URL = {http://www.jstor.org/stable/41000410},
 abstract = {The first goal of this article is to consider influence analysis of principal Hessian directions (pHd) and highlight how such an analysis can provide valuable insight into its behaviour. Such insight includes reasons as to why pHd can sometimes return informative results when it is not expected to do so, and why many prefer a residuals-based pHd method over its response-based counterpart. The secondary goal of this article is to introduce a new influence measure applicable to many dimension reduction methods based on average squared canonical correlations. A general form of this measure is also given, allowing for application to dimension reduction methods other than pHd. A sample version of the measure is considered, with respect to pHd, with two example data sets.},
 author = {L. A. Prendergast and J. A. Smith},
 journal = {{S}cand. {J}. {S}tat.},
 pages = {588--611},
 publisher = {[Board of the Foundation of the Scandinavian Journal of Statistics, Wiley]},
 title = {Influence Functions for Dimension Reduction Methods: An Example Influence Study of Principal Hessian Direction Analysis},
 volume = {37},
 year = {2010}
}% number = {4},

@article{Smith07,
author = {L. A. Prendergast and J. A. Smith},
title = {{Sensitivity of principal Hessian direction analysis}},
volume = {1},
journal = {{E}lectron. {J}. {S}tat.},
publisher = {Institute of Mathematical Statistics and Bernoulli Society},
pages = {253 -- 267},
keywords = {Dimension reduction, influence function, influential observations, principal hessian directions},
year = {2007},
doi = {10.1214/07-EJS064},
URL = {https://doi.org/10.1214/07-EJS064}
}%number = {none},



@article{10.2307/20441398,
 ISSN = {00063444},
 URL = {http://www.jstor.org/stable/20441398},
 abstract = {Sliced inverse regression, sliced inverse regression II and sliced average variance estimation are three related dimension-reduction methods that require relatively mild model assumptions. As an approximation for the relative influence of single observations from large samples, the influence function is used to compare the sensitivity of the three methods to particular observational types. The analysis carried out here helps to explain why there is a lack of agreement concerning the preferability of these dimension-reduction procedures in general. An efficient sample version of the influence function is also developed and evaluated.},
 author = {L. A. Prendergast},
 journal = {Biometrika},
 pages = {585--601},
 publisher = {[Oxford University Press, Biometrika Trust]},
 title = {Implications of Influence Function Analysis for Sliced Inverse Regression and Sliced Average Variance Estimation},
 volume = {94},
 year = {2007}
} %number = {3},

@article{li1989,
author = "{L}i, K.-C. and {D}uan, N.",
doi = "10.1214/aos/1176347254",
fjournal = "The Annals of Statistics",
journal = "{A}nn. {S}tat.",
pages = "1009--1052",
publisher = "The Institute of Mathematical Statistics",
title = "Regression Analysis Under Link Violation",
url = "https://doi.org/10.1214/aos/1176347254",
volume = "17",
year = "1989"
}%number = "3", month = "09",

@article{hall1993,
author = "{H}all, P. and {L}i, K.-C.",
doi = "10.1214/aos/1176349155",
fjournal = "The Annals of Statistics",
journal = "{A}nn. {S}tat.",
pages = "867--889",
publisher = "The Institute of Mathematical Statistics",
title = "On almost Linearity of Low Dimensional Projections from High Dimensional Data",
url = "https://doi.org/10.1214/aos/1176349155",
volume = "21",
year = "1993"
}%number = "2", month = "06",

@article{10.2307/2291214,
 ISSN = {01621459},
 URL = {http://www.jstor.org/stable/2291214},
 abstract = {A framework is developed for the interpretation of regression plots, including plots of the response against selected covariates, residual plots, added-variable plots, and detrended added-variable plots. It is shown that many of the common interpretations associated with these plots can be misleading. The framework also allows for the generalization of standard plots and the development of new plotting paradigms. A paradigm for graphical exploration of regression problems is sketched.},
 author = {R. D. Cook},
 journal = {{J}. {A}m. {S}tat. {A}ssoc.},
 pages = {177--189},
 publisher = {[American Statistical Association, Taylor & Francis, Ltd.]},
 title = {On the Interpretation of Regression Plots},
 volume = {89},
 year = {1994}
} %number = {425},


@article{Cook96,
title = "Graphics for regressions with a binary response",
abstract = "Central dimension-reduction subspaces, which characterize the dependence of a response variable on one or more predictors, are developed and then used to guide the construction and interpretation of graphics for regression problems with a binary response variable. Graphical methods requiring neither a link function nor residuals are suggested for both development and criticism of model components implied by the central dimension-reduction subspace.",
keywords = "Dimension-reduction subspaces, Graphical regression, Logistic regression, Sliced inverse regression",
author = {R. D. Cook},
year = "1996",
day = "1",
doi = "10.1080/01621459.1996.10476968",
language = "English (US)",
volume = "91",
pages = "983--992",
journal = "{J}. {A}m. {S}tat. {A}ssoc.",
issn = "0162-1459",
publisher = "Taylor and Francis Ltd."
}%number = "435",  month = "9",
Access to Document

    10.1080/01621459.1996.10476968

    Link to publication in Scopus
    Link to citation list in Scopus



@article{Lue04,
 ISSN = {00063444},
 URL = {http://www.jstor.org/stable/20441110},
 abstract = {We consider a nonlinear regression problem with predictors with measurement error. We assume that the response is related to unknown linear combinations of a p-dimensional predictor vector through an unknown link function. Instead of observing the predictors, we observe a surrogate vector with the property that its expectation is linearly related to the predictor vector with constant variance. We use an important linear transformation of the surrogates. Based on the transformed variables, we develop the modified Principal Hessian Directions method for estimating the subspace of the effective dimension-reduction space. We derive the asymptotic variances of the modified Principal Hessian Directions estimators. Several examples are reported and comparisons are made with the sliced inverse regression method of Carroll & Li (1992).},
 author = {H.-H. Lue},
 journal = {Biometrika},
 pages = {409--423},
 publisher = {[Oxford University Press, Biometrika Trust]},
 title = {Principal Hessian Directions for Regression with Measurement Error},
 volume = {91},
 year = {2004}
}% number = {2},

@article{article,
author = {Li, Lexin and Cook, R and Nachtsheim, Christopher},
year = {2004},
month = {08},
pages = {175-193},
title = {Cluster-based estimation for sufficient dimension reduction},
volume = {47},
journal = {{C}omput. {S}tat. {D}ata {A}nal.},
doi = {10.1016/j.csda.2003.10.017}
}

@Article{Shaker,
  author   = {Shaker, A. J. and Prendergast, L. A.},
  title    = {Iterative application of dimension reduction methods},
  journal  = {{E}lectron. {J}. {S}tat.},
  year     = {2011},
  volume   = {5},
  pages    = {1471--1494},
  doi      = {10.1214/11-EJS650},
  file     = {:/home/marina/Dropbox/Iterative application.pdf:PDF},
  keywords = {Adaptive estimation, random operator, Inverse problem, oracle inequality, curve alignment, Dimension reduction, Ordinary least squares, sliced inverse regression, Sliced average variance estimation, Principal Hessian directions, cumulative mean estimation, cumulative variance estimation, cumulative directional regression},
}

@article{garnham2013,
author = "Garnham, A. L. and Prendergast, L. A.",
doi = "10.1214/13-EJS831",
fjournal = "Electronic Journal of Statistics",
journal = "{E}lectron. {J}. {S}tat.",
pages = "1983--2004",
publisher = "The Institute of Mathematical Statistics and the Bernoulli Society",
title = "A note on least squares sensitivity in single-index model estimation and the benefits of response transformations",
url = "https://doi.org/10.1214/13-EJS831",
volume = "7",
year = "2013"
}

@article{Prendergast2016ResponseAP,
  title={Response and predictor folding to counter symmetric dependency in dimension reduction},
  author={L.A. Prendergast and A. L Garnham},
  journal={{A}ust. {N}. {Z}. {J}. {S}tat. },
  year={2016},
  volume={58},
  pages={515-532}
}

@article {BR77,
    AUTHOR = {Brillinger, D. R.},
     TITLE = {The identification of a particular nonlinear time series system},
   JOURNAL = {Biometrika},
    VOLUME = {64},
      YEAR = {1977},
     PAGES = {509-515}
} %   NUMBER = {3},



@article{Pearson1901,
author = { K. Pearson  },
title = {On lines and planes of closest fit to systems of points in space},
journal = {{L}ondon, {E}dinburgh {D}ublin {P}hilos. {M}ag. {J}. {S}ci.},
volume = {2},
pages = {559-572},
year  = {1901},
publisher = {Taylor & Francis},
doi = {10.1080/14786440109462720},

URL = { 
        https://doi.org/10.1080/14786440109462720
    
},
eprint = { 
        https://doi.org/10.1080/14786440109462720
    
}

}%number = {11},

@article{10.2307/2290564,
 ISSN = {01621459},
 URL = {http://www.jstor.org/stable/2290564},
 author = {R. D. Cook and S. Weisberg},
 journal = {{J}. {A}m. {S}tat. {A}ssoc.},
 pages = {328--332},
 publisher = {[American Statistical Association, Taylor & Francis, Ltd.]},
 title = {Sliced Inverse Regression for Dimension Reduction: Comment},
 volume = {86},
 year = {1991}
}% number = {414},

@article{PRENDERGAST_2005,
	doi = {10.1111/j.1467-9469.2005.00447.x},
	url = {https://doi.org/10.1111%2Fj.1467-9469.2005.00447.x},
	year = 2005,
	publisher = {Wiley},
	volume = {32},
	pages = {385--404},
	author = {L. A. Prendergast},
	title = {Influence Functions for Sliced Inverse Regression},
	journal = {{S}cand. {J}. {S}tat.}
}%	number = {3}, 	month = {sep},

@article{Pren06,
author = {Prendergast, L. A.},
title = {DETECTING INFLUENTIAL OBSERVATIONS IN SLICED INVERSE REGRESSION ANALYSIS},
journal = {{A}ust. {N}. {Z}. {J}. {S}tat.},
volume = {48},
pages = {285-304},
keywords = {dimension reduction, influence function, influential observations, sliced inverse regression},
doi = {10.1111/j.1467-842X.2006.00441.x},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/j.1467-842X.2006.00441.x},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/j.1467-842X.2006.00441.x},
abstract = {Summary The detection of influential observations on the estimation of the dimension reduction subspace returned by Sliced Inverse Regression (SIR) is considered. Although there are many measures to detect influential observations in related methods such as multiple linear regression, there has been little development in this area with respect to dimension reduction. One particular influence measure for a version of SIR is examined and it is shown, via simulation and example, how this may be used to detect influential observations in practice.},
year = {2006}
}%number = {3},


@article{Benasseni1990,
  title={Sensitivity coefficients for the subspaces spanned by principal components},
  author={B\'{e}nass\'{e}ni, J.},
  journal={{C}ommun. {S}tat. - {T}heory {M}ethods},
  year={1990},
  volume={19},
  pages={2021-2034}
}

@article{Ferre98,
author = { L.   Ferré },
title = {Determining the Dimension in Sliced Inverse Regression and Related Methods},
journal = {{J}. {A}m. {S}tat. {A}ssoc.},
volume = {93},
pages = {132-140},
year  = {1998},
publisher = {Taylor & Francis},
doi = {10.1080/01621459.1998.10474095},

URL = { 
        https://www.tandfonline.com/doi/abs/10.1080/01621459.1998.10474095
    
},
eprint = { 
        https://www.tandfonline.com/doi/pdf/10.1080/01621459.1998.10474095
    
}

}%number = {441},

@article{Pren07,
 ISSN = {00063444},
 URL = {http://www.jstor.org/stable/20441398},
 abstract = {Sliced inverse regression, sliced inverse regression II and sliced average variance estimation are three related dimension-reduction methods that require relatively mild model assumptions. As an approximation for the relative influence of single observations from large samples, the influence function is used to compare the sensitivity of the three methods to particular observational types. The analysis carried out here helps to explain why there is a lack of agreement concerning the preferability of these dimension-reduction procedures in general. An efficient sample version of the influence function is also developed and evaluated.},
 author = {L. A. Prendergast},
 journal = {Biometrika},
 pages = {585--601},
 publisher = {[Oxford University Press, Biometrika Trust]},
 title = {Implications of Influence Function Analysis for Sliced Inverse Regression and Sliced Average Variance Estimation},
 volume = {94},
 year = {2007}
}% number = {3},

@article{prendergast2008a,
author = "Prendergast, L. A.",
doi = "10.1214/08-EJS201",
fjournal = "Electronic Journal of Statistics",
journal = "{E}lectron. {J}. {S}tat.",
pages = "454--467",
publisher = "The Institute of Mathematical Statistics and the Bernoulli Society",
title = "A note on sensitivity of principal component subspaces and the efficient detection of influential observations in high dimensions",
url = "https://doi.org/10.1214/08-EJS201",
volume = "2",
year = "2008",
}%{\GG{20080626}}  {\GG{20080626}} month = "march"

@Article{Prendergast2008,
  author    = {L. A. Prendergast},
  title     = {Trimming influential observations for improved single-index model estimated sufficient summary plots},
  journal   = {{C}omput. {S}tat. {D}ata {A}nal.},
  year      = {2008},
  volume    = {52},
  pages     = {5319--5327},
  doi       = {10.1016/j.csda.2008.05.014},
  file      = {:/home/marina/Dropbox/1-s2.0-S0167947308002806-main.pdf:PDF},
  publisher = {Elsevier {BV}},
}%{\GG{20080803}} %  number    = {12},   month     = {aug},


@article{Cook77,
 ISSN = {00401706},
 URL = {http://www.jstor.org/stable/1268249},
 abstract = {A new measure based on confidence ellipsoids is developed for judging the contribution of each data point to the determination of the least squares estimate of the parameter vector in full rank linear regression models. It is shown that the measure combines information from the studentized residuals and the variances of the residuals and predicted values. Two examples are presented.},
 author = {R. D. Cook},
 journal = {Technometrics},
 pages = {15--18},
 publisher = {[Taylor & Francis, Ltd., American Statistical Association, American Society for Quality]},
 title = {Detection of Influential Observation in Linear Regression},
 volume = {19},
 year = {1977}
}% number = {1},

@article{Li91b,
 ISSN = {01621459},
 URL = {http://www.jstor.org/stable/2290568},
 author = {K.-C. Li},
 journal = {{J}. {A}m. {S}tat. {A}ssoc.},
 pages = {337--342},
 publisher = {[American Statistical Association, Taylor & Francis, Ltd.]},
 title = {Sliced Inverse Regression for Dimension Reduction: Rejoinder},
 volume = {86},
 year = {1991}
} %number = {414},


@article{SHEATHER20081908,
title = {Sliced mean variance–covariance inverse regression},
journal = {{C}omput. {S}tat. {D}ata {A}nal.},
volume = {52},
pages = {1908-1927},
year = {2008},
issn = {0167-9473},
doi = {https://doi.org/10.1016/j.csda.2007.06.007},
url = {https://www.sciencedirect.com/science/article/pii/S0167947307002435},
author = {S. J. Sheather and J. W. McKean and K. Crimin},
keywords = {Classification, Dimension reduction, Discrimination, QR-decomposition, SAVE, SIR, Visualization},
abstract = {Inverse regression methods have gained popularity over the last 10 years or so. More recently these methods have been applied to the classification problem. Sliced inverse regression (SIR) is equivalent to linear discriminant analysis and as such it detects mean differences between the classes. Sliced average variance estimation (SAVE) is designed to detect differences between the means, variances and covariances of the predictors across the classes. However, in SAVE each difference in variance across the groups takes up a dimension, and hence SAVE can have difficulty detecting mean differences and covariance differences. In this paper, we propose a new data analytic method, called sliced mean variance–covariance regression (SMVCIR) which can readily detect both first and second order differences between the classes even when many variance differences exist. Further, our procedure is based on an ordering of the dimensions based on their relative importance which is quite beneficial to interpretation. In particular, we demonstrate that useful data-analytic information about mean and covariance differences can be obtained from SMVCIR when SAVE finds many dimensions due to variance differences. Finally, the advantages of SMVCIR over SIR and SAVE are exemplified using a new data set from the enology literature.}
}%number = {4},

@article{YeWeiss,
author = {Z. Ye and R. E. Weiss},
title = {Using the Bootstrap to Select One of a New Class of Dimension Reduction Methods},
journal = {{J}. {A}m. {S}tat. {A}ssoc.},
volume = {98},
pages = {968-979},
year  = {2003},
publisher = {Taylor & Francis},
doi = {10.1198/016214503000000927},

URL = { 
        https://doi.org/10.1198/016214503000000927
    
},
eprint = { 
        https://doi.org/10.1198/016214503000000927
    
}

}%number = {464},

@article{ZHU20072621,
title = {On hybrid methods of inverse regression-based algorithms},
journal = {{C}omput. {S}tat. {D}ata {A}nal.},
volume = {51},
pages = {2621-2635},
year = {2007},
issn = {0167-9473},
doi = {https://doi.org/10.1016/j.csda.2006.01.005},
url = {https://www.sciencedirect.com/science/article/pii/S0167947306000090},
author = {L.-X. Zhu and M. Ohtaki and Y. Li},
keywords = {Dimension reduction, Sliced inverse regression, Sliced average variance estimation, Hybrid methods},
abstract = {This paper is two-fold. First, we present a further investigation for the hybrid methods of inverse regression-based algorithms. This investigation provides the evidence of how the hybrids gain the advantages to become more powerful methods than the existing methods when the central dimension reduction (CDR) space is estimated. Second, a Bayes Information Criterion (BIC)-type algorithm is recommended to estimate the dimension of the CDR space. Differing from the popularly used sequential test methods, the new algorithm does not require the asymptotic normality of the estimator of the inverse regression-based matrix. The BIC-based estimator is proven to be consistent. A set of simulations for several typical models were carried out to guide the selection of coefficient in the hybrids.}
}%number = {5},

@article{CookLi2002,
author = {R.D. Cook and B. Li},
title = {{Dimension reduction for conditional mean in regression}},
volume = {30},
journal = {{A}nn {S}tat.},
publisher = {Institute of Mathematical Statistics},
pages = {455 -- 474},
keywords = {central subspace, graphics, pHd, regression, SAVE, SIR, visualization},
year = {2002},
doi = {10.1214/aos/1021379861},
URL = {https://doi.org/10.1214/aos/1021379861}
}%number = {2},

@article{Zhu2010,
author = {L.-P. Zhu and L.-X. Zhu and Z.-H. Feng},
title = {Dimension Reduction in Regressions Through Cumulative Slicing Estimation},
journal = {{J}. {A}m. {S}tat. {A}ssoc.},
volume = {105},
pages = {1455-1466},
year  = {2010},
publisher = {Taylor & Francis},
doi = {10.1198/jasa.2010.tm09666},

URL = { 
        https://doi.org/10.1198/jasa.2010.tm09666
    
},
eprint = { 
        https://doi.org/10.1198/jasa.2010.tm09666
    
}

}%number = {492},


@InProceedings{Olive2004,
author="Olive, D. J.",
editor="Hubert, M.,
Pison, G.,
Struyf, A.,
Van Aelst, S.",
title="Visualizing 1D Regression",
booktitle="Theory and Applications of Recent Robust Methods",
year="2004",
publisher="Birkh{\"a}user Basel",
address="Basel, Switzerland",
pages="221--233",
abstract="Regression is the study of the conditional distribution of the response y given the predictors x. In a 1D regression, y is independent of x given a single linear combination $\beta$Tx of the predictors. Special cases of 1D regression include multiple linear regression, binary regression and generalized linear models. If a good estimate b of some non-zero multiple c$\beta$ of $\beta$ can be constructed, then the 1D regression can be visualized with a scatterplot of bTx versus y. A resistant method for estimating c$\beta$ is presented along with applications.",
isbn="978-3-0348-7958-3"
}


@Book{Huber1981,
 Author = {P. J. {Huber}},
 Title = {{Robust statistics}},
 FJournal = {{Wiley Series in Probability and Mathematical Statistics}},
 Journal = {{Wiley Ser. Probab. Math. Stat.}},
 Year = {1981},
 Publisher = {John Wiley \& Sons, Hoboken, NJ},
 Language = {English},
 MSC2010 = {62F35 62-02 62F10},
 Zbl = {0536.62025}
}
